Understanding Zero-Shot Adversarial Robustness for Large-Scale Models

Pretrained large-scale vision-language models like CLIP have exhibited strong generalization over unseen tasks. Yet imperceptible adversarial perturbations can significantly reduce CLIP's performance on new tasks. In this work, we identify and explore the problem of \emph{adapting large-scale models for zero-shot adversarial robustness}. We first identify two key factors during model adaption -- training losses and adaptation methods -- that affect the model's zero-shot adversarial robustness. We then propose a text-guided contrastive adversarial training loss, which aligns the text embeddings and the adversarial visual features with contrastive learning on a small set of training data. We apply this training loss to two adaption methods, model finetuning and visual prompt tuning. We find that visual prompt tuning is more effective in the absence of texts, while finetuning wins in the existence of text guidance. Overall, our approach significantly improves the zero-shot adversarial robustness over CLIP, seeing an average improvement of over 31 points over ImageNet and 15 zero-shot datasets. We hope this work can shed light on understanding the zero-shot adversarial robustness of large-scale models.

==> src/backup.tex <==

Under review as a conference paper at ICLR 2023
TEXT-GUIDED CONTRASTIVE ADVERSARIAL TRAIN-
ING FOR ZERO-SHOT ROBUSTNESS
Anonymous authors
Paper under double-blind review
ABSTRACT
Pretrained large-scale vision-language models have exhibited strong generaliza-
tion over unseen tasks. Yet a small adversarial perturbation can significantly un-
dermine their performance.
There are works that improve models adversarial robustness, however, at a cost of
losing the standard
, leading to serious concerns when deploying the model to safety critical applica-
tions. We observe that the commonly used linear probing is not effective at im-
proving robustness. do not retain models’ (adversarial) robustness for new tasks.
We present Adversarially learned Visual Prompting (AVP), a lightweight approach
to adapting large scale models in the pixel space, to make the model adversarially
robust. More importantly, we show that our learned visual prompt generalizes
to unseen datasets and tasks, improving the models’ zero-shot adversarial robust-
ness. We conduct extensive experiments over 12 zero-shot datasets and find that
AVP improves the adversarial robustness of CLIP in new tasks by an average of
21 points.
1 INTRODUCTION
Large-scale models trained on vision and language data have emerged as a powerful paradigm for
tackling many recognition problems in computer vision and robotics. In addition to state-of-the-
art performance on multiple benchmarks, one of their key advantages is zero-shot generalization,
where the models use just a single textual description to recognize visual categories with high accu-
racy. However, the robustness to adversarial examples remains a challenge, where an imperceptible
pattern can be combined with the image to cause recognition failures.
Due to the importance of this problem, there is a large literature that investigates adversarial ro-
bustness for neural networks. The most common approach for adversarial defense is to modify or
finetune the parameters of the whole model through adversarial training, which mines for adversar-
ial examples and augments the training set with them. While this approach provides robustness to
the target distribution, Radford and Pham established that the same procedure comes at the cost of
generalization. By modifying the weights of the model, the ability to recognize objects from just
textual descriptions becomes significantly degraded.
Existing adversarial methods require finetuning the parameters of the model. However, while this
approach provides robustness on the target distribution, Radford and Pham established that
showed that modifying the weights of the model comes at a cost of generalization. To defend against
adversarial examples, the existing methods require finetuning the model on a target distribution.
Adversarial training backfires on CLIP because modifying the weights destroys the zero-shot gener-
alization. If we use adversarial training for robustness on zero-shot tasks, we consequently lose the
ability to do zero-shot tasks.
In this paper, we defend against adversarial examples by modifying the inputs of the model instead of
the parameters of the model. The natural language processing community has found that many tasks
can be solved by designing the right input prompt, and these techniques have extended to the visual
domain as well. Instead of finetuning the parameters of the network, our approach finds a visual
prompt that is added to the input image and that instructs the model to be robust against adversarial
1
Under review as a conference paper at ICLR 2023
attacks. Since we only modify the input, this defense strategy consequently allows the representation
to transfer to new problems and maintain strong zero-shot generalization performance.
Talk about experiments.
Talk about contribu







\begin{table}[t]
\centering
\caption{Zero-shot robust accuracy training on CIFAR100 \xin{main results}}
% \vspace{-3mm}
    \begin{tabular}{cl|cccccc}
         \toprule
        %  & \multicolumn{6}{c}{DRN-22-d} \\
         & & \multicolumn{6}{c}{Number of Training Categories}\\
         
         & Method  & 15  & 30 & 45 & 60  &  75 & 90 \\
        %  \midrule 
        %   & {ImageNet} & \\
         \midrule
         & Trained Categories CLIP& & 7.03 & 7.03 & 4.68 & 6.05 & 7.42\\
         & Trained Categories  Ours & 78.13 & 69.14 & 51.37& 61.72 & 58.98 & 54.69\\
         & Non-overlap Categories CLIP \\
         & Non-overlap Categories Ours \\
         
         
         &CIFAR10 &  & 10.16 & 10.16 & \\
         & CIFAR10 Ours& 32.62 & 47.46 & 51.37 & 51.36 & 44.53 & 47.07\\
         \midrule
         
         \bottomrule
    \end{tabular}
\vspace{-2mm}
\label{tab:targeted}
\end{table}


\begin{table}[t]
\centering
\caption{Zero-shot CLEAN accuracy training on CIFAR100}
% \vspace{-3mm}
    \begin{tabular}{cl|cccccc}
         \toprule
        %  & \multicolumn{6}{c}{DRN-22-d} \\
         & & \multicolumn{6}{c}{Number of Training Categories}\\
         
         & Method  & 15  & 30 & 45 & 60  &  75 & 90 \\
        %  \midrule 
        %   & {ImageNet} & \\
         \midrule
         & CIFAR100 Trained Categories CLIP & 69.53  & 66.41 & 67.97 & 65.43 & 62.50& 66.41\\
         & CIFAR100  Trained Categories  Ours & 89.45  & 82.81 & 82.81 & 81.64 & 76.76 & 75.19\\
         & CIFAR100 New Categories CLIP & \\
         & CIFAR100  New Categories  Ours & \\
          
         &CIFAR10 & 88.28 &  \\
         & CIFAR10 Ours & 62.11 & 73.63 & 70.90& 70.51 & 61.32 & 62.89\\
         \midrule
         
         \bottomrule
    \end{tabular}
\vspace{-2mm}
\label{tab:targeted}
\end{table}







\begin{table}[t]
\centering
\caption{Zero-shot robust accuracy}
\adjustbox{width=\linewidth}{
% \vspace{-3mm}
    \begin{tabular}{cl|llllllllll}
         \toprule
        %  & \multicolumn{6}{c}{DRN-22-d} \\
         & & \multicolumn{6}{c}{Method} \\
         \midrule
        %  & & \multicolumn{3}{c|}{Baselines} & \multicolumn{3}{c}{Our Prompting} \\
         
         & PGD 100  & CLIP & LP & VP & AFT (scott) & AFT(Contrastive) & AFT(img contrastive) & AFT Ours& Visual Prompt (onehot) & Visual Prompt (contrastive) & Visual Prompt (img contrastive)  \\
        %  \midrule 
        %   & {ImageNet} & \\
         \midrule
         \parbox[t]{1mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{Zero-Shot Test Tasks}}} & ImageNet* & 0 & & & &45.12 \\
         & CIFAR10 & 9.59 && 13.25 & 59.41 &  \\
         & STL-10 & 35.40 && 40.74 &  & \\
         & CIFAR100 & 4.55 && 5.59  & 34.12 &  \\
         & SUN & 1.02 & &1.60 & 29.55 & \\
         & StanfordCars & 0.27 && 0.21 & 13.54 & \\
         & Food101 & 3.95 && 4.21 & 28.15 & \\
         & OxfordPet & 2.72 && 3.24  & 60.62 & \\
         & Flower102 & 1.19&& 1.77 & 31.56 & \\
         & Country211 & 0.09& & 0.06 & 3.28 &   \\
         & DTD & 2.5&& 3.56 & 22.82 &   \\
         & EUROSAT & 0.04 && 0.01 & 14.48 &  \\
         & FGVC & 0.00 && 0.00 & 5.31 &  \\
         & HatefulMemes &  &&  & 31.30 &  &  & 23.12 \\
         & PatchCamelyon &  &&  & 22.42 &  &  & \\
         & Caltech101 &  &  && 0.82 &  &  & \\
         & Caltech256 &  &  && 0.82 &  &  & \\

         \midrule
         & Average & 5.11 & & & & 26.46 & 26.25\\
         
         
         \bottomrule
    \end{tabular}}
\vspace{-2mm}
\label{tab:targeted} % add LP, AFT under parameters constrain, adding propt to AFT best.
\end{table}

\begin{table}[t]
\centering
\caption{Zero-shot robust accuracy \xin{main results}}
\adjustbox{width=\linewidth}{
% \vspace{-3mm}
    \begin{tabular}{cl|lll|lll}
         \toprule
        %  & \multicolumn{6}{c}{DRN-22-d} \\
         & & \multicolumn{6}{c}{Method} \\
         \midrule
         & & \multicolumn{3}{c|}{Baselines} & \multicolumn{3}{c}{Our Prompting} \\
         
         & PGD 100  & CLIP  & VP & AFT & Added & Appended  & Appended  \\
         & Training Set Labeled & Yes & Yes & Yes  & Yes & Yes & No \\
        %  \midrule 
        %   & {ImageNet} & \\
         \midrule
         \parbox[t]{1mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{Zero-Shot Test Tasks}}} & ImageNet* &\\
         & CIFAR10 & 9.59 & 13.25 & 59.41 & 33.36 & 49.18&  48.73 \\
         & STL-10 & 35.40 & 40.74 &  & 57.42 & 75.54 & 75.43 \\
         & CIFAR100 & 4.55 & 5.59  & 34.12 & 14.84 & 25.82 & 24.82\\
         & SUN & 1.02 & 1.60 & 29.55 & 10.82 & 24.87 & 22.58 \\
         & StanfordCars & 0.27 & 0.21 & 13.54 & 3.78 &10.91 & 12.05 \\
         & Food101 & 3.95& 4.21 & 28.15 &7.45 & 20.10 & 20.38 \\
         & OxfordPet & 2.72 & 3.24  & 60.62 &23.63 &48.57& 47.26\\
         & Flower102 & 1.19& 1.77 & 31.56 & 12.36 & 23.73 & 24.54\\
         & Country211 & 0.09 & 0.06 & 3.28 & 0.63 & 2.43 & 2.04 \\
         & DTD & 2.5& 3.56 & 22.82 & 14.09 & 21.11 & 21.22 \\
         & EUROSAT & 0.04 & 0.01 & 14.48 & 0.35  & 11.26 & 12.49\\
         & FGVC & 0.00 & 0.00 & 5.31 &1.77 & 4.05 & 3.48 \\
         & HatefulMemes &  &  & 31.30 &  &  &  \\
         & PatchCamelyon &  &  & 22.42 &  &  & \\
         & Caltech101 &  &  & 0.82 &  &  & \\
         & Caltech256 &  &  & 0.82 &  &  & \\

         \midrule
         & Average & 5.11 & & & & 26.46 & 26.25\\
         
         
         \bottomrule
    \end{tabular}}
\vspace{-2mm}
\label{tab:targeted}
\end{table}





\begin{table}[t]
\centering
\caption{Zero-shot clean accuracy}
% \vspace{-3mm}
\adjustbox{width=\linewidth}{
    \begin{tabular}{cl|llllll}
         \toprule
        %  & \multicolumn{6}{c}{DRN-22-d} \\
         & & \multicolumn{6}{c}{Method} \\
         
         & Clean  & CLIP  & VP & AFT & Ours (add) & Ours  & Ours (unlabeled)  \\
        %  \midrule 
        %   & {ImageNet} & \\
         \midrule
         \parbox[t]{1mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{Zero-Shot Test Tasks}}} & ImageNet* &\\
         & CIFAR10 &  89.06 & 86.72 & 78.40 & 61.29 & 71.63 & 70.65 \\
         & STL-10 &  97.16 & 95.90 & & 88.40 & 91.59 & 91.31\\
         & CIFAR100 & 62.32 & 59.35 & 49.81 & 30.82 & 40.96  & 39.41 \\
         & SUN397 & 57.67 & 59.08 & 51.95 & 41.61 & 50.97 & 47.27 \\
         & StanfordCars & 52.14 & 47.61 & 34.13 & 27.36 & 33.50 & 37.87  \\
         & Food101 & 83.15 & 76.74 & 56.52 & 41.92 & 52.41 & 55.39 \\
         & OxfordPet & 85.82 & 85.91 & 81.39 & 71.92 & 79.07 & 78.25 \\
         & Flower102 & 65.64 & 60.48 & 52.15 & 39.34 &45.78 & 46.17 \\
         & Country211 & 15.25 & 12.80 & 8.27 & 4.93 &7.41 & 6.91 \\
         & DTD & 40.53 & 12.81 & 34.10 & 29.73 &31.86 & 32.44\\
         & EUROSAT & 38.26 & 33.85 & 25.69 & 10.29 &15.93 & 19.47 \\
         & FGVC & 20.04 & 19.05 & 13.53 & 10.80 &12.24 & 12.69 \\
         & HatefulMemes &  &  & 53.37 &  &  & \\
         & PatchCamelyon &  &  & 49.63 &  &  & \\
         & Caltech101 &  &  &  &  &  & \\
         & Caltech256 &  &  &  &  &  & \\
         \midrule
         & Average & &&&& 44.45 &44.82 \\
         \bottomrule
    \end{tabular}}
\vspace{-2mm}
\label{tab:targeted}
\end{table}








%%%Unlabeled


\begin{table}[t]
\centering
\caption{\small{Are labels required to adapt large-scale models for zero-shot adversarial robustness?}}
\adjustbox{width=\linewidth}{
% \vspace{-3mm}
    \begin{tabular}{cl|llllllllllllllll}
         \toprule
        %  & \multicolumn{6}{c}{DRN-22-d} \\
         & & \multicolumn{6}{c}{Method} \\
         \midrule
        %  & & \multicolumn{3}{c|}{Baselines} & \multicolumn{3}{c}{Our Prompting} \\
         
         & PGD 100  & ImageNet & {CIFAR10} & STL-10 & CIFAR100 & SUN & StanfordCars & Food101 & OxfordPet & Flower102 & DTD & EUROSAT & FGVC & HatefulMemes & PatchCamelyon & Caltech101 & Caltech256 \\
        %  \midrule 
        %   & {ImageNet} & \\
         \midrule
         VPT Robust Accuracy & Labeled & 23.71 & 49.18 & 75.54 & 25.82 & 24.87 & 10.91 & 20.10 & 48.57 & 23.73& 21.11 & 11.26 & 4.05 & 31.13 & 30.50 & 63.79 & 47.66 \\
         VPT Robust Accuracy & Unlabeled &   23.79 & 48.73 & 75.43 & 24.83 & 22.58 & 12.05 & 20.38 & 47.26 & 24.54 & 21.22 & 12.49 & 3.48 & 26.40 & 40.22 & 65.55 & 49.41 \\ %cv12, right bottom
         
         \midrule
         VPT Clean Accuracy & Labeled & 48.84& 71.63 & 91.59 & 40.96 & 50.97 & 33.50 & 52.41 & 79.07 & 45.78 & 31.86 & 15.93 & 12.24 & 58.53 & 47.85 &  95.19 & 71.66 \\
         VPT Clean Accuracy & Unlabeled & 59.11 & 70.65 & 91.31 & 39.41 & 47.27 & 37.87 & 55.39 & 78.25 & 46.17 & 32.44 & 19.47 & 12.69 & 55.83 & 49.60 & 86.34 & 73.60\\
         
         \midrule
         AFT Robust Accuracy & Labeled &  41.88 & 59.28 & 83.45 & 34.13 & 29.81 & 13.37 & 27.99 & 62.61 & 30.69 & 22.88 & 15.18 & 5.10 & 31.97 & 23.87 & 69.07 & 59.54 \\
         AFT Robust Accuracy & Unlabeled & 38.76 & 60.90 & 79.41 & 31.56 & 30.33 & 13.87 & 27.72 & 58.84 & 29.48 & 22.50 & 11.67 & 5.10 & 29.97 & 19.14 & 67.49 & 59.41 \\ % cv12, w2
         
         \midrule
         AFT Clean Accuracy & Labeled & 63.87 & 78.12 & 93.30 & 49.68 & 51.28 & 33.30 & 55.37 & 81.58 & 50.92 & 34.15 & 27.57 & 13.89 & 53.47 & 49.01 & 83.51 & 76.51\\
         AFT Clean Accuracy & Unlabeled & 58.87 & 80.51 & 91.18 & 49.08 & 54.93 & 39.39 & 59.14 & 77.62 & 50.79 & 34.20 & 26.13 & 14.52 & 52.10 & 52.97 & 81.39 & 77.93 \\
         
         \bottomrule
    \end{tabular}}
\vspace{-2mm}
\label{tab:unlabeled} % add LP, AFT under parameters constrain, adding propt to AFT best.
\end{table}


